Exploring Bi-Manual Teleportation in Virtual Reality

Teleportation, a widely-used locomotion technique in Virtual Reality (VR), allows instantaneous movement within VR environments. Enhanced hand tracking in modern VR headsets has popularized hands-only teleportation methods, which eliminate the need for physical controllers. However, these techniques have not fully explored the potential of bi-manual input, where each hand plays a distinct role in teleportation: one controls the teleportation point and the other confirms selections. Additionally, the influence of users' posture, whether sitting or standing, on these techniques remains unexplored. Furthermore, previous teleportation evaluations lacked assessments based on established human motor models such as Fitts' Law. To address these gaps, we conducted a user study (N=20) to evaluate bi-manual pointing performance in VR teleportation tasks, considering both sitting and standing postures. We proposed a variation of the Fitts' Law model to accurately assess users' teleportation performance. We designed and evaluated various bi-manual teleportation techniques, comparing them to uni-manual and dwell-based techniques. Results showed that bi-manual techniques, particularly when the dominant hand is used for pointing and the non-dominant hand for selection, enable faster teleportation compared to other methods. Furthermore, bi-manual and dwell techniques proved significantly more accurate than uni-manual teleportation. Moreover, our proposed Fitts' Law variation more accurately predicted users' teleportation performance compared to existing models. Finally, we developed a set of guidelines for designers to enhance VR teleportation experiences and optimize user interactions.

==> X4_implementation.tex <==
\section{Implementation}

\outline{Explains implementations in detail - commonly used for hardware related papers, etc.}

\subsection{Hardware}
\outline{present the device and hardware used}
%Smartwatch LEMFO LEM7 Android 7, a 1.3GHz CPU and a 2MP side camera and \todo{vision angle}.

% We employed the Oculus Quest Pro VR headset for its integrated cameras and the Oculus Hand Tracking SDK for hand tracking instead of marker-based or external motion tracking solutions. Unity 3D (2020.3.33f1) was the primary development software used, with C# scripting to design and create the techniques and virtual environment. The Oculus Integration SDK was utilized to access real-time tracking data on key points on the users' hands, such as their palm and finger joints. Oculus Wireless Link was employed for rapid development on a computer with RTX 3070 GPU. The data logged during study sessions was automatically transferred from the headset to a Cloud-Firestore database.






==> xDontUse01_abstract.tex <==
Abstract goes here

maximum 150 word abstract (aim for ~120)

30 word contribution statement (used for final version, but good to write now)




